Efficient Data Race Detection of Async-Finish Programs Using Vector Clocks

Existing data race detectors for task-based programs incur significant run time and space overheads. The overheads arise because of frequent lookups in fine-grained tree data structures to check whether two accesses can happen in parallel. This work shows how to efficiently apply vector clocks for dynamic data race detection of async-finish programs with locks. Our proposed technique, FastRacer, builds on the FastTrack algorithm with per-task and per-variable optimizations to reduce the size of vector clocks. FastRacer exploits the structured parallelism of async-finish programs to use a coarse-grained encoding of the dynamic task inheritance relations to limit the metadata in the presence of many concurrent readers. Our evaluation shows that FastRacer substantially improves time and space overheads over FastTrack, and is competitive with the state-of-the-art data race detectors for async-finish programs with locks.

==> chktexrc <==
# see /usr/local/texlive/*/texmf-dist/chktex/chktexrc for all defaults

# call like `chktex -v2 -g -l ~/.chktexrc paper.tex` to get local config to overwrite global

# if you get the message, "WARNING -- ChkTeX does not handle lines over 1021 bytes correctly",
# you might find this regular expression handy: [^\n]{1021,}

# supposedly this is the default and it's in the global chktexrc but doesn't work unless repeated here
# QuoteStyle = Traditional #=> "An example," he said, "would be great."
# QuoteStyle = Logical     #=> "An example", he said, "would be great".
QuoteStyle = Logical

TabSize = 2

# -v2 means fancy error display
# but for some reason we can't use it here; it has to go before the other command line options, i.e., -g
# CmdLine
# {
#     -v
# }

# Allow only "-" and "---" separators inside words
HyphDash
{
    1 3
}

# Allow only "--" separators between numbers (the global default)
NumDash
{
    2
}

# Disallow all usage of " --- ", " -- ", or " - "
WordDash
{
    0
}

# ignore "Command terminated with space" warnings for these commands:
Silent
{
    \begingroup
    \centering
    \dash
    \dots
    \draw
    \endgroup
    \endinput
    \footnotemark
    \hfil
    \hfill
    \item
    \ldots
    \linebreak
    \makeappendix
    \makeatletter
    \makeatother
    \maketableofcontents
    \maketitle
    \medskip
    \newline
    \node
    \noindent
    \path
    \phantomsection
    \printbibliography
    \quad
    \today
# math operators
    \approx
    \geq
    \neg
    \supset
    \wedge
# size commands
    \tiny
    \scriptsize
    \footnotesize
    \small
    \normalsize
    \large
    \Large
    \LARGE
    \huge
    \Huge
# booktabs
    \bottomrule
    \midrule
    \toprule
# caption/subcaption/subfig packages
    \ContinuedFloat
}


==> fastpar-pseudocode-merged-algorithmic.tex <==
\begin{small}
	\begin{algorithm}[H]
		\caption{\small \fastpar analysis at synchronization operations}
		\label{alg:fastpar-sync-ops}
		\begin{algorithmic}[1]
			% \Procedure{Spawn}{}
			\STATE \COMMENT{Task \task{T} spawns task \task{U}}

			\IF{\texttt{size}(\task{T.rw\_vc}) $>$ \textsf{THRESHOLD}}
			\STATE \task{T.ro\_vc} $\leftarrow$ REF(\{\task{T.ro\_vc} $\cup$ \task{T.rw\_vc}\})
			\STATE \task{T.rw\_vc} $\leftarrow$ $\emptyset$
			\ENDIF

			\STATE \task{U.ro\_vc} $\leftarrow$ \task{T.ro\_vc}
			\STATE \task{U.rw\_vc} $\leftarrow$ \task{T.rw\_vc} $\cup$ \{\task{T.epoch}\}
			\STATE \task{U.joined} $\leftarrow$ \task{T.joined}

			\STATE \task{T.epoch} $\leftarrow$ \task{T.epoch} + 1
			\STATE \task{U.epoch} $\leftarrow$ \task{U.epoch} + 1
			%		\State \algorithmiccomment{incrementEpoch() function creates a new epoch with clock value incremented by 1 and returns its pointer.}
			% \EndProcedure
		\end{algorithmic}

		\begin{algorithmic}[1]
			% \Procedure{Join}{}
			\STATE \COMMENT{Task \task{T} joins with \task{U}}
			\STATE \task{T.joined} $\leftarrow$ \task{T.joined} $\cup$ \{\texttt{getTaskId}(\task{U.epoch})\}
			% \State \algorithmiccomment{getTaskId() function returns TaskId of the corresponding epoch}
			% \EndProcedure
		\end{algorithmic}

		\begin{algorithmic}[1]
			% \Function{CheckHB}{\epoch{c}{u},\task{T}}
			\STATE \COMMENT{Check HB between epoch \epoch{c}{u} and current access by \task{T}}
			\IF{\epoch{c}{u} $\preceq$ \task{T.rw\_vc} \textbf{or} c@u $\preceq$ \task{T.ro\_vc} \textbf{or} \task{u} $\in$ \task{T.joined}}
			\STATE \RETURN true
			\ENDIF
			\STATE \RETURN false
			% \EndFunction
		\end{algorithmic}
	\end{algorithm}
\end{small}


==> fastpar-pseudocode.tex <==
\begin{small}
	% \begin{minipage}{0.46\textwidth}
	\begin{algorithm}[H]
		\caption{\hfill \fastpar: Task \task{T} spawns task \thr{U}}
		\label{alg:fastpar-task-spawn-opt}
		\begin{algorithmic}[1]
			\If{\texttt{size}(T.rw\_vc) $>$ THRESHOLD}
			\State T.ro\_vc $\gets$ REF(\{T.ro\_vc $\cup$ T.rw\_vc\})
			\State T.rw\_vc $\gets$ $\emptyset$
			\EndIf

			\State U.ro\_vc $\gets$ T.ro\_vc
			\State U.rw\_vc $\gets$ T.rw\_vc $\cup$ \{T.epoch\}
			\State U.joined $\gets$ T.joined
			%                \State U.m\_rw\_vc $\gets$ T.m\_rw\_vc $\cup$ \{<T.taskid , T.clock>\}
			%           \State U.wait\_rovc $\gets$ T.spawn\_rovc
			%           \State U.wait\_rwvc $\gets$ T.spawn\_rwvc $\cup$ \{<T.taskid , T.clock>\}

			\State T.epoch $\gets$ T.epoch + 1
			\State U.epoch $\gets$ U.epoch + 1
			%		\State \algorithmiccomment{incrementEpoch() function creates a new epoch with clock value incremented by 1 and returns its pointer.}
		\end{algorithmic}
	\end{algorithm}

	\begin{algorithm}[H]
		\caption{\hfill \fastpar: Task \thr{T} joins with Task \thr{U}}
		\label{alg:fastpar-join-opt}
		\begin{algorithmic}[1]
			\State T.joined  $\gets$ T.joined $\cup$ \{getTaskId(U.epoch)\}
			\State \algorithmiccomment{getTaskId() function returns TaskId of the corresponding epoch}
			%
			%           \ForAll{<t,c> in U.wait\_rwvc}
			%           \State vc $\gets$ \{T.wait\_rovc $\cup$ T.wait\_rwvc\}
			%           \State T.wait\_rwvc[t]$\gets$max(U.wait\_rwvc[t],vc[t])
			%           \State T.spawn\_rwvc[t]$\gets$max(U.wait\_rwvc[t],vc[t])
			%           \EndFor
		\end{algorithmic}
	\end{algorithm}
	% \end{minipage}
	% \hspace{5pt}
	% \begin{minipage}{0.46\textwidth}
	\begin{algorithm}[H]
		\caption{\hfill \fastpar: HB\_Check(c@u,\thr{T})}
		\label{alg:fastpar-hb-check}
		\begin{algorithmic}[1]
			\If{c@u $\preceq$ \thr{T}.rw\_vc \textbf{or} c@u $\preceq$ \thr{T}.ro\_vc \textbf{or} u $\in$ \thr{T}.joined }
			\State \textbf{return} true
			\EndIf
			\State \textbf{return} false
		\end{algorithmic}
	\end{algorithm}

	% \begin{algorithm}[H]
	% 	\caption{\hfill \fastpar: Task \thr{T} acquires Lock L}
	% 	\label{alg:fastpar-lockAcquire}
	% 	\begin{algorithmic}[1]
	% 		\State T.lockset $\gets$ T.lockset $\cup$ \{L\}
	% 	\end{algorithmic}
	% \end{algorithm}

	% \begin{algorithm}[H]
	% 	\caption{\hfill \fastpar: Task \thr{T} releases Lock L}
	% 	\label{alg:fastpar-lockRelease}
	% 	\begin{algorithmic}[1]
	% 		\State T.lockset $\gets$ T.lockset $\setminus$ \{L\}
	% 	\end{algorithmic}
	% \end{algorithm}

	% \end{minipage}
\end{small}


==> fastpar.tex <==
\section{\fastpar: Specializing %Efficient
  Dynamic Data Race Detection for \pcode{Async-Finish} Programs}
\label{sec:new-algo}

In this section, we present \emph{\fastpar}, a novel algorithm that exploits the structured parallelism of \pcode{async-finish} programs for efficient data race detection.
% \fastpar uses epochs and vector clocks to check whether two accesses happen in parallel or not (\pcode{\small CHECKHB (Algorithm \ref{alg:nft-CHECKHB})}).
\fastpar is essentially an adaptation of \nft for \pcode{async-finish} programs;
all the optimizations discussed for \nft are included in \fastpar.
% Similar to above, task vector clock is divided into \pcode{ro\_vc}, \pcode{rw\_vc} and \pcode{joinset} and \pcode{\small CHECKHB} checks HB relationship against all three.
\Fastpar differs from \nft in (i) how locks are handled and (ii) variable metadata are maintained. While \nft uses vector clocks to track lock acquire and release (like \ft), \fastpar uses the lockset mechanism~\cite{eraser} for handling locks. Every task in \fastpar maintains a lockset, \ie, the set of locks held by the task, and updates the lockset at lock acquire and release operations.
%  instead of updating the vector clock.
\NFT maintains all concurrent readers that access a shared variable which can be large for task-based programs.
% , affecting the performance.
\fastpar uses coarse-grained tracking of dynamic task inheritance relationships
% instead of the finer-grained DPST data structure
to select few accesses from parallel readers/writers\footnote{When tasks use locks,
    two writes can happen in parallel but still not constitute a race if they are protected by the same lock.},
which allows it to maintain constant metadata per-lockset per-variable.
\FASTPAR continues to use vector clocks for race detection.
% \FastPar exploits structured parallelism of \pcode{async-finish} programs to further improve the performance of data race detection. \FASTPAR continues to use vector clocks for race detection but maintains constant metadata per-lockset per-variable.
% Furthermore, \fastpar uses coarse-grained tracking of dynamic task inheritance relationships instead of the finer-grained DPST data structure to select concurrent readers/writers.
These insights allow \fastpar to outperform \cracer, \ptracer, and \nft (\Cref*{sec:eval:perf}).

% Optimizations discussed in Section~\ref{sec:nft-design} allow the \ft to run for task parallel
% programs. Even though the \nft algorithm is applicable to a much wider range of programs than
% async-finish, still \nft performs comparably to \ptracer. To further improve the performance of
% data race detection of \pcode{async-finish} programs, we exploit the structured nature of these
% programs. Here we introduce \fastpar, a novel algorithm for data race detection of
% \pcode{async-finish} programs. All the optimizations discussed for \nft are applicable for the
% metadata maintained per task, but the metadata maintained per variable can still grow large in the
% case of shared reads and writes, as \nft maintains full vector clocks for these cases. While
% \ptracer maintains constant metadata per-lockset per-variable due to the enforced ordering of
% nodes during the creation of a DPST, and can be more space efficient than the vector clock
% representation of \nft. The performance bottleneck in \ptracer is in finding the LCA of different
% \pcode{step} nodes because of the large size of a DPST. \fastpar uses vector clocks for data race
% detection and maintains constant metadata per lockset per variable using the concept of
% \emph{inheritance vector clocks}. These insights allow \fastpar to outperform both \ptracer and
% \nft.

% \NFT is a significant improvement for task-based programs over the \naive \ft algorithm (Section~\ref{sec:eval:perf}). However, the size of the vector clocks can still be large for applications with a pathological sequence of updates to shared variables. Our insight to improve the performance of dynamic data race detection of task-based programs further is that the different approaches have advantages when viewed in isolation. For example, \PTRACER maintains constant metadata per-lockset per-variable due to the enforced ordering of nodes during creation of a DPST, and can be more space efficient than the vector clock representation of \nft. The performance bottleneck in \ptracer is in finding the LCA of different \pcode{step} nodes because of the large size of a DPST. Vector clocks allow \nft to efficiently check for data races (excepting the \rdshared and \wrshared states) compared to the LCA computation in \ptracer, which can be expensive if the DPST is deep.
% We propose a novel algorithm \emph{\fastpar} which uses vector clocks for data race detection and maintains constant metadata per lockset per variable using the concept of \emph{inheritance vector clocks}. These insights allow \fastpar to outperform both \ptracer and \nft.

% \paragraph*{Key insight}
%
%\nft is essentially an optimized version of \ft, using vector clocks for Data Race Detection. Vector clocks help \nft checking for race in constant time, except Read Shared and Write Shared case, in which it is of the order of number parallel reads. Since, in task-parallel program, there are huge number of parallel tasks, \nft bears large time and memory overhead even after applying all State and Task optimizations. On the other hand, \ptracer maintains constant metadata per lockset per variable, using DPST and so does away with the issue of Read and Write Shared case of \nft. However, \ptracer computes LCA between different nodes to check for race between them, which takes a lot of time due to large depth of DPST. \\
%We hereby propose a novel algorithm \fastpar which uses Vector Clocks for Data Race Detection and maintains constant metadata per lockset per variable using Vector Clock Representation of Inheritance tree i.e. \textit{Inheritance Vector Clock} This helps \fastpar performing all race checks in constant time and is able to outperform both \nft and \ptracer.\\
%

% In Section~\ref{sec:motivation}, we discussed the advantages and disadvantages of vector clock and task graph based techniques.
% \NFT is essentially an optimized vector-clock-based data race detector for task parallel programs which allows it to have better run-time and memory performance than \ft.


% In spite of optimizations specific to task-based programs, \nft continues to incur more run-time and space overhead compared to \ptracer (Section~\ref{sec:eval}). Our insight to improve the performance of dynamic data race detection further is that both the techniques have advantages when viewed in isolation. Vector clocks allow \nft to efficiently check for data races (excepting the \rdshared and \wrshared states) compared to the LCA computation in \ptracer, which can be expensive if the DPST is deep. \PTRACER maintains constant metadata per-lockset per-variable due to the enforced ordering of nodes during creation of a DPST, and so is more space efficient than the vector clock representation of \nft.
% The performance bottleneck in \ptracer is in finding the LCA of different \pcode{step} nodes because of the large size of a DPST. These motivated us to use a different representation, inheritance trees, to model the dynamic inheritance between tasks.
% We propose a novel algorithm \emph{\fastpar} which uses vector clocks for data race detection and maintains constant metadata per lockset per variable using the concept of \textit{inheritance vector clocks}. Our insight allows \fastpar to significantly outperform both \ptracer and \nft.

% This helps \fastpar performing all race checks in constant time and so is able to outperform both \nft and \ptracer.

% \swarnendu{What is the motivation of inheritance vector clocks? Is it encoding similar information compared to a DPST? What is the data structure capturing at a high level?}

% \nft is essentially an optimized version of \ft, using vector clocks for Data Race Detection. Vector clocks help \nft checking for race in constant time, except Read Shared and Write Shared case, in which it is of the order of number parallel reads. Since, in task-parallel program, there are huge number of parallel tasks, \nft bears large time and memory overhead even after applying all State and Task optimizations. On the other hand, \ptracer maintains constant metadata per lockset per variable, using DPST and so does away with the issue of Read and Write Shared case of \nft. However, \ptracer computes LCA between different nodes to check for race between them, which takes a lot of time due to large depth of DPST. \\
% We hereby propose a novel algorithm \fastpar which uses Vector Clocks for Data Race Detection and maintains constant metdata per lockset per variable using \textit{Inheritance Vector Clock}. This helps \fastpar performing all race checks in constant time and so is able to outperform both \nft and \ptracer.

\begin{figure}
    \centering
    \includegraphics[scale=0.40]{inheritance-tree.pdf}
    %    \Description{The inheritance tree corresponding the task-based program in Figure~\ref{fig:task-parallel-code}.}
    \caption{The inheritance tree corresponding the task-based program in Figure~\ref{fig:task-parallel-code}.}
    \label{fig:inheritance-graph}
\end{figure}

\subsection{Maintaining Constant Per-Variable Metadata}
\label{sec:constant-metadata}

\FastPar models the dynamic parent-child relationship among the different tasks created in a program with a \emph{task inheritance} tree. The nodes represent tasks, and edges represent the creation of child tasks by the parent. When a task \task{T1} creates a child task \task{T2}, an edge \task{T1} \(\rightarrow\) \task{T2} is added to the tree. Figure~\ref{fig:inheritance-graph} shows the inheritance tree for the task-based program shown in Figure~\ref{fig:task-parallel-code} (ignore the IVC labels for now).

%\shivam{R2: If I understood the Tusker algorithm correctly, I don't see how it can detect races correctly.  The key optimization it has done on the inheritance tree loses enough information that I don't see how certain cases of series-parallel relationships can be maintained correctly.}

\paragraph*{Maintaining constant per-variable metadata}

% The goal of using an inheritance tree in \fastpar is similar to using DPST in \ptracer.
The metadata stored per shared variable in \fastpar is proportional to the number of the different locksets with which the variable has been accessed.
\FastPar uses the inheritance tree to \emph{efficiently} select two accesses out of multiple concurrent accesses with the same lockset, such that any racy future access which races with any one of the concurrent accesses must be racy with either one of the two chosen last accesses.
% The same holds true for the Inheritance tree as well i.e.
For parallel tasks accessing a variable with the same lockset, \fastpar stores the access
history of the two tasks with the highest LCA in the inheritance tree (\Cref*{lemma:one}).
% \shivam{Review this line about LCA}
% \shivam{Here, it's assumed that Fig1 is updated, with T3 spawning Tasks T4 and T5, and both T4 and T5 write to var1 proected by lock}
Consider the three accesses to \code{var1} from tasks \task{T2}, \task{T4}, and \task{T5} in \Cref{fig:task-parallel-code}.
In the inheritance tree shown in Figure~\ref{fig:inheritance-graph},
%  corresponding to example code in Figure~\ref{fig:task-parallel-code}
task nodes \task{T2} and \task{T4} (or \task{T5}) have the highest LCA, and so we store the access
histories from \task{T2} and \task{T4} and discard \task{T5}. Any further access to \code{var1}, which is not parallel with both \task{T2} and \task{T4}, will not be parallel with \task{T5} as well. So, discarding \task{T5}'s access information is sound.\footnote{In \pcode{\smaller async-finish} semantics, a task must join with its ancestor, either immediate or recursive. In case a parent task calls \pcode{\smaller join}, all children tasks within this join scope, either immediate or recursive, join with it.}

Similar to \fastpar, \ptracer selects two accesses out of multiple concurrent accesses with the same lockset using a specific tree called DPST.
The primary difference between a DPST used in \ptracer\cite{ptracer-fse-2016} and an inheritance tree is in the \emph{granularity} of the nodes.
While a DPST breaks up a task into several unsynchronized regions represented by \pcode{step} nodes, an inheritance tree has just one node per task. The coarser modeling makes the inheritance tree much smaller and shallower compared to the DPST. Also, unlike a DPST, there is no left-to-right ordering in an inheritance tree.
While \ptracer uses DPST to check the concurrency between two accesses and select accesses with the highest LCA, \fastpar only does the latter with the inheritance tree. \fastpar continues to use \nft's vector clocks for data race detection to compensate for the coarser modeling and loss of ordering between the nodes.

\paragraph*{Inheritance vector clock}

% \swarnendu{What exactly is the difference between a task inheritance tree and the IVC?}

% \hilite{\fastpar doesn't build \textit{Inheritance tree} but instead uses it's idea of selecting two accesses out of multiple concurrent accesses. \fastpar uses a data structure called \textit{Inheritance Vector Clock} to select the accesses with highest LCA in the tree and so no tree traversal is done to compute it. This is unlike \ptracer, which actually builds and traverses DPST to compute LCA.}
% \swarnendu{I think we are repeating the fact that inheritance trees are used for constant metadata quite a few times.}

While \ptracer actually builds a DPST and traverses it repeatedly to compute LCAs, \fastpar, instead of building Inheritance Tree, encodes the inheritance relationship in a per-task array of clock values
% called \emph{Inheritance Vector Clock} (IVC)
for better performance.
% \textcolor{red}{\fastpar uses an \emph{inheritance vector clock} (IVC) to encode the dynamic parent-child relationships among tasks.}
An \emph{Inheritance Vector Clock} (IVC)
is a per-task immutable vector clock
% that remains unchanged during the lifetime of the task. An IVC
that contains the clock values of all the %recursive
reachable parents of a task \task{T} at the time of the creation of \task{T}. An IVC identifies the unique path in the inheritance tree from the root task to \task{T}, since a task spawn increments the scalar clock of the caller task. Whenever a parent task creates a child task, \fastpar copies the parent's IVC to the child and appends the parent's current clock value at the end of child IVC. In Figure~\ref{fig:inheritance-graph}, the IVC of the parent task \task{T3} is copied to the child task \task{T4} and the current clock of \task{T3} (assumed to be one) is appended.

\FastPar's IVC labeling is similar to Offset-Span (OS) labeling~\cite{mellor-crumney-sc-1991}.
Both the schemes
compute a unique label from the label of the immediate predecessor, and guarantee that the length of a task's label will always be proportional to the
% nesting depth of current fork-join pair, \ie, the
depth of the task in the inheritance tree.
However, there are two differences. % between the schemes.
First, the IVC of a task, once created, is immutable. Unlike OS labeling, any further task join operations do not modify the IVC. Second, the IVC label can be dynamically computed.
% while building the task graph itself.
The Span part of OS labeling can only be assigned after the task graph is completed, \ie, OS labels cannot be computed while building the task graph. Intuitively,
IVC labels are more similar to the Offset part,
% of OS labeling,
with the constraint that they do not
get updated at \pcode{join} operations.
% Note that \fastpar could do away with this relaxation
% without compromising on the correctness because
Whereas prior work~\cite{mellor-crumney-sc-1991} uses OS labels for race detection, \fastpar uses IVC labels to identify two accesses out of multiple parallel accesses having the highest LCA in the inheritance tree.
% \sout{For race detection, \fastpar continues to use the \nft
%     % vector clock
%     algorithm.}

%  and thus correctness is ensured.

% \shivam{I used term fork-join above. Is it okay?}
% \shivam{The clain that OS labels can't be computed dynamically while building the taskgraph isn't written in the paper, but it's quite easy to infer. They just say that it's similar to English-Hebrew modelling}
%\shivam{R2: The IVC labeling scheme is very similar to the scheme proposed by John Mellor-Crummey from his work in 91 [32]}

% We have used \textit{Inheritance Vector Clock} for modeling parent-child relationships among the tasks created. IVC is a PerTask ReadOnly Vector Clock, which remains constant during the lifetime of the task. It actually contains the clock values of all the recursive parents of the task, at the time of creation of task and uniquely identifies the thread in the Inheritance tree from root to the the task.(See Fig ???) Whenever a parent task creates a child task, we copy the IVC of parent to child and append the parent's current clock value at the end of child IVC.

%\swarnendu{Say how an inheritance tree is different from Offset-Span labeling.}

\paragraph*{Computing tasks with highest LCA}
\label{lca-computation}

To compute the highest LCA among three parallel tasks, \fastpar iterates over the IVCs of all the tasks simultaneously and stops at the first point of difference. Thereafter, \fastpar chooses the task with a different clock value and any one of the other two. If all the three clock values are different, any two out of three tasks can be chosen. If \fastpar reaches the end of an IVC for any task \task{T}, that indicates that \task{T} must be the parent of the other two in the inheritance tree, and so, \fastpar chooses the parent task \task{T} and any one from the other two. The tasks so chosen will have the highest LCA in the inheritance tree (see \Cref*{lemma:two})
% and so correctness is ensured.

% \swarnendu{Shivam: From the above description, it is not clear what would happen if all three IVCs have different clock values at the same index.}

In the example shown in Figure~\ref{fig:task-parallel-code}, the accesses to the variable \code{var1} from three parallel tasks, \task{T2},\task{T4}, and \task{T5}, are with the same lockset \code{\{L1\}}. The IVCs of the corresponding task nodes,
% in the inheritance tree,
shown in Figure~\ref{fig:inheritance-graph}, are IVC$_{T2}$=[1], IVC$_{T4}$ = [2,1], and IVC$_{T5}$ = [2,2].
To select two out of the three accesses, \fastpar iterates over the three IVCs simultaneously. The first point of difference is at the first entry itself: IVC$_{T2}$[0]=1, IVC$_{T4}$[0]=IVC$_{T5}$[0]=2. So, \fastpar selects a task with a different clock value, \ie, \task{T2} and any one of other two, say \task{T4} (or \task{T5}). For the given example, tasks \task{T2} and \task{T4} (or \task{T5}) indeed have the highest LCA in the inheritance tree.

% \shivam{I am getting some errors in compiling to make T2 subscript in IVCT2, please fix this}
% For finding the tasks with highest LCA among three parallel tasks, we iterate over the IVC of all the tasks simultaneously and stop at the first point of difference. Thereby we choose the task with different clock value and any one of other two. If we reach to the end of IVC for any task, that denotes the considered task is the parent of other two in the Inheritance tree and so, we choose that parent task and any two of other. The tasks so chosen will have the highest LCA in the Inheritance tree and so correctness is ensured.

The computation overhead depends on the sizes of the IVC, which is equal to the height of the inheritance tree. Since an inheritance tree is much shallower compared to a DPST, the computation is relatively efficient.
% \sout{Finally, using the IVC allows \fastpar to maintain constant metadata per variable per lockset by zeroing in on the accesses of tasks with the highest LCA in the inheritance tree.}

% The time overhead of this computation will be of the order of size of IVC, which is equal to the depth of the task in Inheritance tree. Since Inheritance tree is much shallower as compared to DPST, the computation is highly efficient. Finally using the IVC, we maintain constant metadata per variable per lockset by selecting the accesses of Tasks with highest LCA in the Inheritance tree.
% \shivam{Do we need to define what LCA is? as it's done in ptracer paper for DPST}

%\subsection{Data Race Checks}
%We use \ft VectorClock Operations to check happens-before relationship between two accesses. For all race-checks, we need to compare the access history of the variable with the clock value of the task in current task metadata. This helps us reducing the time computation of race checks to O(1).
%At every variable access, we compare the last access clock value with the clock value of the last task in current TaskState. If the former is greater, as per \ft rules, we have racy condition, otherwise we update the variable metadata accordingly.

\subsection{Detecting Data Races}
\label{sec:fastpar:data-races}

At the core of \FastPar is a vector-clock-based data race detection algorithm based on \nft.

% \sout{At the core of \FastPar is a vector-clock-based data race detection algorithm. Inspired by the metadata efficiency of DPST-based techniques, \fastpar uses the IVC to maintain constant per-variable metadata for each distinct set of locks held during a memory access. This is in addition to \nft vector clocks for having race detection. In other words, \fastpar optimizes the overhead of the \rdshared and the \wrshared states in \nft.}

% Furthermore, all the optimizations that are part of \nft are included in \fastpar, which allows it to outperform both \ptracer and \nft (Section~\ref{sec:eval}).

% \fastpar inherits Vector Clock Structure from \ft and lock handling algorithm from ptracer. Thereafter, using the \textit{Inheritance Vector Clock} we maintain constant perVariable metadata for each distinct set of locks held before access. Also, all optimizations suggested in \nft are also incorporated in it, making it finally outperform all the above algorithms.

\savespace{
    \input{fig-fastpar-metadata-state.tex}
}

\paragraph*{Metadata structure}

\FastPar extends the per-task metadata maintained in \nft with two attributes: \pcode{lockset} tracks the set of locks held by a task, and \pcode{IVC} helps maintain constant per-variable metadata.
The per-variable metadata in \fastpar is an array of lock metadata. Each lock metadata stores
the access history of the variable with the distinct set of locks held before the
access. Every per-lock metadata contains four access history entries, two each for
reads and writes, which contain the epoch value and a reference to the IVC of the task at the time
of access.
%  In total,
% \sout{Every lock metadata contains four epochs and four references to IVCs of the corresponding tasks.}
Storing references to the IVCs suffice since they remain unchanged during the lifetime of a task.

% Each task \task{T} contains its own epoch value in \code{epoch} and the vector clock is broken into a read-only part \code{ro\_vc} and a read-write part \code{rw\_vc}. Each task \task{T} maintains the set of tasks that have already joined with \task{T}
% the current task
% in \code{joinset} and an extra \code{IVC} attribute to help \fastpar maintain constant per variable metadata.

% The per-task metadata maintained in \fastpar is shown in \Cref{fig:fastpar-metadata-states}, and is similar to \nft. Each task \task{T} contains its own epoch value in \code{epoch} and the vector clock is broken into a read-only part \code{ro\_vc} and a read-write part \code{rw\_vc}. Each task \task{T} maintains the set of tasks that have already joined with \task{T}
% % the current task
% in \code{joinset} and an extra \code{IVC} attribute to help \fastpar maintain constant per variable metadata.

%
%
% maintains two vector clocks, storing the clock values of other tasks that \task{T} has synchronized with. Maintaining two vector clocks, as in \nft, allows \fastpar to be efficient during the \pcode{spawn()} and \pcode{join()} calls (Section~\ref{sec:nft-design}).
%
%\swarnendu{This is vague.}
%\shivam{is it clear now?}

% \fastpar Task Metadata structure and operations are identical to that of \nft. Every Task has an associated TaskState, which has Double VC, containing the clock values of other tasks synchronized with it. Double VC form, as \nft, helps \fastpar optimizing the time and space overhead in spawn as well as wait calls.(Section ~\ref{sec:design}) However, Task Vector Clocks are not updated in case of lockAcquire and
% lockRelease. Instead, every TaskState has a lockset containing the set of locks acquired by the tasks at any time.So, in every lockAcquire the lock is added to the Task lockset, and in lockRelease, the lock is removed from the lockset. Therefore, \fastpar manages lock operations in O(1) time.

%\swarnendu{SK: What is ``int lockset'' in PerLockMetadata?}

% PerVariable Metadata in \fastpar is actually an array of lockStates, with every lockState storing access history to the variable with a distinct set of locks held before the access(lockset). Further,every lockstate contains four access history entries, two for reads and two for writes, which constitute of epoch value and reference to \textit{Inheritance Vector Clock}(IVC) of the task at the time of access. Therefore every lockstate contains total 4 epochs: R1, R2, W1 and W2, and reference to IVC of corresponding tasks: IR1, IR2, IW1 and IW2.(See Fig2) Note here, that since Task IVC remains unchanged during the lifetime of the task, and so storing the reference doesn't create any correctness issues.

\savespace{
    \input{fig-fastpar-racecheck-algo.tex}
}

\paragraph*{Race checks}

\fastpar iterates over all the lock metadata corresponding to distinct locksets with which a shared memory variable has been accessed. An empty intersection of the lockset of the current access and the lock metadata implies potentially parallel accesses. If the two locksets are disjoint, \FastPar checks if the epoch values stored in the access history happens before the current access using vector clocks (\pcode{\smaller CHECKHB}, \Cref*{alg:fastpar-sync-ops}).
% The function \pcode{CheckHB} in Algorithm~\ref{alg:fastpar-sync-ops} shows how \fastpar uses vector clocks and \pcode{joinset} to check for the happens-before relationship between past accesses and the current access.
If there is no such relationship, it implies that the prior access is concurrent with the current access. Finally, \fastpar reports a data race if one of the two accesses is a write.

% Algorithm~\ref{alg:fastpar-racecheck-algo} shows the steps executed by \fastpar to check for data races on an access to a shared memory variable. \fastpar iterates over all the lock metadata corresponding to distinct locksets with which the variable has been accessed and checks if the intersection of the lockset of the current access and lock metadata is empty (lines 3--4). If the two locksets are disjoint, which implies potential parallel accesses, \FastPar checks if the epoch values stored in the access history happens before the current access using vector clocks.
%(similar to \nft).
% \fastpar uses \nft vector clocks (and joinset) to check for the happens-before relationship between past accesses and the current access (see Algorithm ~\ref{alg:fastpar-hb-check}). If there is no such relationship, it implies that the prior access is concurrent with the current access. Finally, if one of the two accesses is a write, \fastpar reports a data race.

% Figure~\ref{fig:fastpar-racecheck-algo} provides the algorithm for checking the metadata on shared memory access. In every such access, the algorithm iterates over all the lockstates corresponding to distinct locksets with which the variable has been accessed. First it checks if the intersection of the lockset of current access and lockstate is empty, if true that means current access may be parallel with the access entries of the lockstate. So, we check if the epoch value of the access entries happen before the current Task VectorClock otherwise the access entry is concurrent with current access. Finally, if one of the two accesses are write, the algorithm reports the data race.

\paragraph*{Metadata updates}

If a read does not race with prior writes, then \fastpar updates the read metadata corresponding to the current lockset. \FastPar checks if any of the read epochs in the lock metadata corresponding to the current lockset happens before the current task's access using vector clocks.
% (Algorithm ~\ref{alg:fastpar-sync-ops}).
If yes, then \FastPar updates that access entry with the current task's epoch and IVC. Otherwise, there are three parallel reads, and \fastpar needs to select two with the highest LCA. \FastPar iterates over the IVC of all three access entries and stops either at the first point of difference or if one of the IVCs end. \fastpar stores the access history of the task corresponding to selected IVC and any one of the other two. Using any one of the other two works since, in both the cases, the two chosen tasks will have the highest LCA in the inheritance tree (Section~\ref{lca computation}).
% \paragraph*{Metadata update example}
Figure~\ref{fig:tusker-example1} shows an example of how \fastpar updates the read metadata.
% Let's consider an example (see Figure~\ref{fig:tusker-example1}) for \fastpar read metadata updation.
Assume tasks \task{T2}, \task{T3}, and \task{T4} all read a shared variable \code{x} and task
\task{T5} writes \code{x}. After the reads from \task{T2} and \task{T3}, the two readers stored for the variable \code{x} are \task{T2} and \task{T3}, because both these tasks can run in parallel.
Since task \task{T4} is spawned by \task{T1} after \task{T1} synchronizes with \task{T2}, so the
read by \task{T4} happens after the read of \task{T2}. The read metadata entry of \task{T2} is
replaced by \task{T4}. Next, when \task{T5} writes \code{x}, \fastpar checks the access with all
previous reads and reports a read-write race between the accesses from \task{T4} and \task{T5}.
%\anupam{R1: If it doesn't matter which of the other two reads are stored, why do you bother storing two reads at all?}
%\shivam{Resolved?}
The steps performed by \fastpar on a write access are similar.

% \hilite{
% % While \nft stores one writer and multiple concurrent readers for each shared variable, \fastpar stores two readers and two writers per lockset.
% Maintaining two reads and two writes per lockset enables \fastpar to detect races both in the current schedule as well as in other schedules for a given input. The behavior is similar to that of \ptracer.
% On the other hand, \nft, similar to \ft, is able to detect races only in the current schedule.
% }
% Therefore, \fastpar uses \nft algorithm for data race detection and Inheritance Vector Clock to store constant metadata per lockset per variable.

%\anupam{Include an algorithm or a paragraph explaining lockAcquire and lockRelease operations.}

\paragraph*{Synchronization operations}

The metadata updates in case of task spawn and join operations are similar to \nft. During a \pcode{spawn} operation (Algorithm~\ref{alg:fastpar-sync-ops}), \fastpar checks if the size of \pcode{rw\_vc} is greater than a threshold. If yes, \fastpar merges \pcode{ro\_vc} and \pcode{rw\_vc} of the parent task into a new \pcode{ro\_vc} for the child task and \pcode{rw\_vc} of the child is kept empty. Otherwise, the child \pcode{ro\_vc} references the parent \pcode{ro\_vc}, and the child \pcode{rw\_vc} is copied from parent \pcode{rw\_vc}. Thereafter, \fastpar copies the parent's \pcode{joinset} and \pcode{lockset}
to the child's \pcode{joinset} and \pcode{lockset} respectively.
% In case of task spawn, \fastpar checks if size of \code{rw\_vc} is less than a threshold, otherwise \fastpar merges \code{ro\_vc} and \code{rw\_vc} into a new \code{ro\_vc} and clears the contents of \code{rw\_vc}. Thereafter, \fastpar copies the \code{ro\_vc} of parent task to child \code{ro\_vc}, \code{rw\_vc} to child \code{rw\_vc} and \code{joinset} to child \code{joinset} (Algorithm ~\ref{alg:fastpar-sync-ops}).
In case of a \pcode{join} operation, the \pcode{joinset} of the parent task is updated to contain the id of the child task, similar to \nft (Algorithm ~\ref{alg:fastpar-sync-ops}).

In case of a lock acquire and release, a task's vector clock is not updated in \fastpar unlike \nft. Instead, \fastpar uses \ptracer's mechanism to deal with lock operations. Each task maintains a \pcode{lockset}.
%  which is the set of locks held by the tasks at any time~\cite{eraser}.
When a task \task{T} acquires a lock \pcode{L}, the \pcode{lockset} of \task{T} is updated to contain lock \pcode{L}. In case of a lock release, \pcode{L} is removed from the lockset.
% (Algorithms ~\ref{alg:fastpar-lockAcquire}--\ref{alg:fastpar-lockRelease}).
When \task{T} accesses a shared variable \code{x}, the \pcode{lockset} is copied to variable metadata. During a race check, \fastpar checks for the intersection of the locksets from the metadata history to infer a data race.

%A task's vector clocks are not updated during synchronization operations. Instead, \fastpar uses \ptracer's mechanism to deal with synchronization operations. Each task maintains a lockset which is the set of locks held by the tasks at any time.
%% So, in every lockAcquire the lock is added to the Task lockset, and in lockRelease, the lock is removed from the lockset.
%At lock acquire and release operations, instead of updating the task's vector clock, \fastpar updates the lockset of the task and the lockset is copied to all relevant variable metadata. During a race check, \fastpar checks for the intersection of the locksets from the metadata history to infer a data race.

% If current access is not found to be racy with all the access entries in the Variable metadata, then metadata corresponding to current lockset needs to be updated. If the current access is read, then we check if any of the read epochs in the lockstate corresponding to current lockset happen before current Task Vector Clock, if true we just update that access entry with current task epoch and IVC. Otherwise, we would have three parallel reads and we need to select the two with highest LCA. So, we iterate over the IVC of all three accesses, and stop either at the first point of difference or if one of them ends. If the IVC that differed or ended is the current Task IVC, we keep the current access history and any one of other two. Otherwise, we leave the metadata unchanged.

% \paragraph*{Write metadata updates.}

% If the race check fails and the current access is write, then we need to update the write metadata of the corresponding lockset. Similar to read case, we check if any of the write epochs in the lockstate corresponding to current lockset happen before current Task VectorClock, if true we update that entr with current Task epoch and IVC. Otherwise we have three parallel writes. Note that this isn't a race, since they are protected by the same lockset. So, similar to read update, we iterate over IVC of all three accesses, and if the task which differed or whose IVC ended first is the current task, we keep the current access history and any two of the other two. Otherwise, we leave the metadata unchanged.

% \swarnendu{\Cref*{alg:fastpar-sync-ops} does not talk about locksets.}

In practice, variables are accessed with the same set of locks, and hence maintaining access metadata for different sets of unique locks is reasonable. Furthermore, metadata update operations depend on the size of the IVC, but we find that the maximum depth of the inheritance tree is small ($\leq 30$ for our benchmarks).

% Thereby maintaining only two reads and writes per lockset help \fastpar perform the race checks in time proportional to the the number of different locksets with which the variable is accessed. In practice, it's observed that the shared variables are accessed with similar locksets and so overall the race check time for \fastpar becomes nearly constant. Also, metdata update operations are of the order of the size of IVC i.e. depth of Inheritance tree, but again in practice, the maximum depth of inheritance tree is found to be very small(< 30 for our benchmarks). Therefore, all VariableMetadata Operations can be done efficiently in \fastpar, which is also verified by the results in Fig ???

\begin{figure}[t]
    \centering
    \begin{subfigure}{.25\linewidth}
        \centering
        \includegraphics[scale=0.55]{figs/tusker-example1-code.pdf}
        \label{fig:example1-code}
    \end{subfigure}%
    % \hspace*{-7em}
    \begin{subfigure}{.7\linewidth}
        \centering
        \includegraphics[scale=0.5]{figs/tusker-example1-ivc.pdf}
        \label{fig:example1-ivc}
    \end{subfigure}
    %    \Description{An example task parallel program with five tasks \task{T1}--\task{T5} to help show how \fastpar captures \pcode{finish} scope.}
    \caption{An \pcode{async-finish} program with five tasks \task{T1}--\task{T5} and the corresponding inheritance tree.}
    \label{fig:tusker-example1}
\end{figure}

\iftoggle{ieeeFormat}{
    % \input{fastpar-pseudocode-merged-algorithmic.tex}
    \input{fastpar-pseudocode-merged-algpseudocode.tex}
}{}

\iftoggle{acmFormat}{
    \input{fastpar-pseudocode-merged-algpseudocode.tex}
}{}

\input{fastpar-lemmas.tex}


==> fig-fastpar-metadata-state.tex <==
\iffalse
    \begin{figure}
        \label{fig:fastpar-metadata}
        \centering
        \begin{lstlisting}[style=CPPStyle]
// Metadata maintained per shared variable
class PerVariableMetadata {
    // Pointers to locks held during an access
    PerLockState L[];
}
// Metadata maintained per lock variable
class PerLockState {
    int lockset_id;
    int r1_tid; // task_id of first reader
    int r1_c; // clock value of first reader
    // pointer to task state of first reader
    PerTaskMetadata* RT1;
    int r2_tid; // task_id of second reader
    int r2_c; // clock value of second reader
    // pointer to task state of second reader
    PerTaskMetadata* RT2;
    int w1_tid; // task_id of first writer
    int w1_c; // clock value of first writer
    // pointer to task state of first writer
    PerTaskMetadata* WT1;
    int w2_tid; // task_id of second writer
    int w2_c; // clock value of second writer
    // pointer to task state of second writer
    PerTaskMetadata* WT2;
}
// Metadata maintained per logical task
class PerTaskMetadata {
    int task_id;
    int scalar_clock;
    int lockset_id;
    map<taskid, int> VC[]; // Task vactor clock
    // Refers to read-only root_vc
    RootVC* root_vc = NULL;
    map<taskid, int> VC2[]; // Task vactor clock
    // Refers to read-only root_vc
    RootVC* root_vc2 = NULL;
}

    \end{lstlisting}
        \anupam{give better names to task vector clocks}
        \caption{Metadata state maintained in \fastpar.}
        \label{fig:metadata-states}
    \end{figure}
\fi

\begin{figure}
    \centering
    \begin{lstlisting}[style=CPPStyle]
class PerVariableMetadata {
    // Pointers to locks held during a memory access
    PerLockMetadata lock[];
}
class PerLockMetadata {
    set<lockID> lockset;
    epoch rd1, rd2;    // Reader 1 and 2 metadata
    IVC* rd1_ivc, rd2_ivc; // IVC of Reader 1 and 2
    epoch wr1, wr2;    // Writer 1 and 2 metadata
    IVC* wr1_ivc,wr2_ivc; // IVC of Writer 1 and 2
}
class PerTaskMetadata {
    epoch epoch;
    map<taskid, clock> ro_vc; // Rd-only vector clock
    map<taskid, clock> rw_vc; // Rd-wr vector clock
    set<taskid> joined;  // All joined child tasks
    set<lockId> lockset; // Locks held by the task
    int IVC[];
}\end{lstlisting}
    % \swarnendu{SK: Does the PerTaskMetadata not have an IVC in addition to what \nft has?}
    \caption{Metadata state maintained in \fastpar.}
    \label{fig:fastpar-metadata-states}
\end{figure}


==> ft-pseudocode-merged-algorithmic.tex <==
\begin{small}

    \begin{algorithm}[ht]

        \caption{\small \FT analysis at synchronization operations}
        \label{alg:ft-sync-ops}
        \begin{algorithmic}[1]
            % \Function{Spawn}{}
            \STATE \thr{U.vc} $\leftarrow$ \thr{T.vc} $\cup$ \{\thr{T.epoch}\}
            \COMMENT{Thread \thr{T} spawns \thr{U}}

            \STATE \thr{T.epoch} $\leftarrow$ \thr{T.epoch} + 1
            \COMMENT{Increment thread's scalar clock}
            \STATE \thr{U.epoch} $\leftarrow$ \thr{U.epoch} + 1
            % \EndFunction
        \end{algorithmic}

        \begin{algorithmic}[1]
            % \Procedure{Join}{}
            \STATE \COMMENT{Thread \thr{T} joins with \thr{U}}
            \FORALL{<t,c> in \thr{U.vc}}
            \STATE \thr{T.vc[t]} $\leftarrow$ \texttt{max}(\thr{U.vc[t]}, \thr{T.vc[t]})
            \ENDFOR
            % \EndProcedure
        \end{algorithmic}

        \begin{algorithmic}[1]
            % \Procedure{Acquire}{}
            \STATE \COMMENT{\thr{T} acquires lock \thr{L}}
            \FORALL{<t,c> in \pcode{L.vc}}
            \STATE \thr{T.vc[t]} $\leftarrow$ \texttt{max}(\pcode{L.vc[t]}, \thr{T.vc[t]})
            \ENDFOR
            % \EndProcedure
        \end{algorithmic}

        \begin{algorithmic}[1]
            % \Procedure{Release}{}
            \STATE \COMMENT{\thr{T} releases lock \thr{L}}
            \STATE \pcode{L.vc} $\leftarrow$ \thr{T.vc}
            \STATE \thr{T.epoch} $\leftarrow$ \thr{T.epoch} + 1
            % \EndProcedure
        \end{algorithmic}

        \begin{algorithmic}[1]
            % \Function{CheckHB}{\epoch{c}{u},\thr{T}}
            \STATE \COMMENT{Check HB between epoch \epoch{c}{u} and current access by \thr{T}}
            \IF{\epoch{c}{u} $\preceq$ \thr{T}.vc}
            \STATE \RETURN true
            \ENDIF
            \STATE \RETURN false
            % \EndFunction
        \end{algorithmic}
    \end{algorithm}
\end{small}


==> ft-pseudocode.tex <==
\begin{small}
    \begin{algorithm}[H]
        \swarnendu{Refer to the Algorithms in prose.}
        \caption{\hfill \ft: Thread \thr{T} spawns \thr{U}}
        \label{alg:ft-task-spawn-unopt}
        \begin{algorithmic}[1]
            % \State \thr{U}.vc $\gets$ \thr{T}.vc
            \State \thr{U}.vc $\gets$ \thr{T}.vc $\cup$ \{\thr{T}.epoch\}
            %\State U.m\_vc $\gets$ U.m\_vc $\cup$ \{<T.taskid , T.clock>\}
            %                \State T.clock $\gets$ T.clock + 1
            %                \State U.clock $\gets$ U.clock + 1
            \State \thr{T}.epoch $\gets$ \thr{T}.epoch + 1
            \State \thr{U}.epoch $\gets$ \thr{U}.epoch + 1
        \end{algorithmic}
    \end{algorithm}
    \begin{algorithm}[H]
        \caption{\hfill \ft: Thread \thr{T} joins with \thr{U}}
        \label{alg:ft-join-unopt}
        \begin{algorithmic}[1]
            \ForAll{<t,c> in \thr{U}.vc}
            \State \thr{T}.vc[t] $\gets$ max(\thr{U}.vc[t], \thr{T}.vc[t])
            \EndFor
        \end{algorithmic}
    \end{algorithm}
    \begin{algorithm}[H]
        \caption{\hfill \ft: HB\_Check(c@u,\thr{T})}
        \label{alg:ft-hb-check}
        \begin{algorithmic}[1]
            \If{c@u $\preceq$ \thr{T}.vc}
            \State \textbf{return} true
            \EndIf
            \State \textbf{return} false
        \end{algorithmic}
    \end{algorithm}
    \begin{algorithm}[H]
        \caption{\hfill \ft: \thr{T} acquires lock \thr{L}}
        \label{alg:ft-lockAcquire}
        \begin{algorithmic}[1]
            \ForAll{<t,c> in \code{L}.vc}
            \State \thr{T}.vc[t] $\gets$ max(\code{L}.vc[t], \thr{T}.vc[t])
            \EndFor
        \end{algorithmic}
    \end{algorithm}
    \begin{algorithm}[H]
        \caption{\hfill \ft: \thr{T} releases lock \thr{L}}
        \label{alg:ft-lockRelease}
        \begin{algorithmic}[1]
            \State \code{L}.vc $\gets$ \thr{T}.vc
            \State \thr{T}.epoch $\gets$ \thr{T}.epoch + 1
        \end{algorithmic}
    \end{algorithm}
\end{small}


==> nft-pseudocode-merged-algorithmic.tex <==
\begin{small}
    \begin{algorithm}[H]
        \caption{\small \NFT analysis at synchronization operations}
        \label{alg:nft-sync-ops}
        \begin{algorithmic}[1]
            \STATE \COMMENT{Task \task{T} spawns \task{U}}
            \IF{\texttt{size}(\task{T.rw\_vc}) $>$ \textsf{THRESHOLD}}
            \STATE \task{U.ro\_vc} $\leftarrow$ REF(\{\task{T.ro\_vc} $\cup$ \task{T.rw\_vc}\})
            \STATE \task{U.rw\_vc} $\leftarrow$ $\emptyset$
            \ELSE
            \STATE \task{U.ro\_vc} $\leftarrow$ \task{T.ro\_vc}
            \STATE \task{U.rw\_vc} $\leftarrow$ \task{T.rw\_vc}
            \ENDIF

            \STATE \task{U.rw\_vc} $\leftarrow$ \task{U.rw\_vc} $\cup$ \{\task{T.epoch}\}
            \STATE \task{U.joinset} $\leftarrow$ \task{T.joinset}

            % \State U.m\_rw\_vc $\gets$ T.m\_rw\_vc $\cup$ \{<T.taskid , T.clock>\}
            % \State U.wait\_rovc $\gets$ T.spawn\_rovc
            % \State U.wait\_rwvc $\gets$ T.spawn\_rwvc $\cup$ \{<T.taskid , T.clock>\}

            % \swarnendu{Is incrementEpoch() different from just incrementing the clock value?}

            % \STATE \algorithmiccomment{incrementEpoch() creates a new epoch with clock value incremented by 1}
            % %  and returns its pointer}
            \STATE \task{T.epoch} $\leftarrow$ \task{T.epoch} + 1
            \STATE \task{U.epoch} $\leftarrow$ \task{U.epoch} + 1
        \end{algorithmic}

        \begin{algorithmic}[1]
            \STATE \COMMENT{Task \task{T} joins with \task{U}}
            \STATE \task{T.joinset} $\leftarrow$ \task{T.joinset} $\cup$ \{\texttt{getTaskId}(\task{U.epoch})\}
            \STATE \COMMENT{\texttt{getTaskId()} returns task id of the corresponding epoch}
            %
            %           \ForAll{<t,c> in U.wait\_rwvc}
            %           \State vc $\gets$ \{T.wait\_rovc $\cup$ T.wait\_rwvc\}
            %           \State T.wait\_rwvc[t]$\gets$max(U.wait\_rwvc[t],vc[t])
            %           \State T.spawn\_rwvc[t]$\gets$max(U.wait\_rwvc[t],vc[t])
            %           \EndFor
        \end{algorithmic}

        \begin{algorithmic}[1]
            \label{alg:nft-CHECKHB}
            % \Function{CheckHB}{\epoch{c}{u},\task{T}}
            \STATE \COMMENT{Check HB between epoch \epoch{c}{u} and current access by \task{T}}
            \IF{\epoch{c}{u} $\preceq$ \task{T.rw\_vc} \textbf{or} \epoch{c}{u} $\preceq$ \task{T.ro\_vc} \textbf{or} \task{u} $\in$ \task{T.joinset}}
            \STATE \RETURN true
            \ENDIF
            \STATE \RETURN false
        \end{algorithmic}
    \end{algorithm}

    %\begin{algorithm}[H]
    %	\caption{\hfill \ft: \thr{T} acquires lock \thr{L}}
    %	\label{alg:ft-lockAcquire}
    %	\begin{algorithmic}[1]
    %		\ForAll{<t,c> in L.vc}
    %		\State T.vc[t] $\gets$ max(L.vc[t], T.vc[t])
    %		\EndFor
    %	\end{algorithmic}
    %\end{algorithm}
    %\begin{algorithm}[H]
    %	\caption{\hfill \ft: \thr{T} releases lock \thr{L}}
    %	\label{alg:ft-lockRelease}
    %	\begin{algorithmic}[1]
    %		\State L.vc $\gets$ T.vc
    %		\State T.m\_epoch $\gets$ T.m\_epoch + 1
    %	\end{algorithmic}
    %\end{algorithm}
\end{small}


==> nft-pseudocode-merged-algpseudocode.tex <==
\begin{small}
    \begin{algorithm}[H]
        \caption{\small \NFT analysis at synchronization operations}
        \label{alg:nft-sync-ops}
        \begin{algorithmic}[1]

            \Procedure{Spawn}{}
            \Comment{Task \task{T} spawns \task{U}}
            \If{\texttt{size}(\task{T.rw\_vc}) $>$ \textsf{\smaller THRESHOLD}}
            \State \task{U.ro\_vc} $\gets$ REF(\{\task{T.ro\_vc} $\cup$ \task{T.rw\_vc}\})
            \State \task{U.rw\_vc} $\gets$ $\emptyset$
            \Else
            \State \task{U.ro\_vc} $\gets$ \task{T.ro\_vc}
            \State \task{U.rw\_vc} $\gets$ \task{T.rw\_vc}
            \EndIf

            \State \task{U.rw\_vc} $\gets$ \task{U.rw\_vc} $\cup$ \{\task{T.epoch}\}
            \State \task{U.joinset} $\gets$ \task{T.joinset}

            % \swarnendu{Is incrementEpoch() different from just incrementing the clock value?}

            % \State \algorithmiccomment{incrementEpoch() creates a new epoch with clock value incremented by 1}
            %  and returns its pointer}
            \State \task{T.epoch} $\gets$ \task{T.epoch} + 1
            \State \task{U.epoch} $\gets$ \task{U.epoch} + 1
            \EndProcedure

            \Procedure{Join}{}
            \Comment{Task \task{T} joins with \task{U}}
            \State \task{T.joinset} $\gets$ \task{T.joinset} $\cup$ \{\texttt{getTaskId}(\task{U.epoch})\}
            % \State \Comment{\texttt{getTaskId()} returns task id of the corresponding epoch}

            %
            %           \ForAll{<t,c> in U.wait\_rwvc}
            %           \State vc $\gets$ \{T.wait\_rovc $\cup$ T.wait\_rwvc\}
            %           \State T.wait\_rwvc[t]$\gets$max(U.wait\_rwvc[t],vc[t])
            %           \State T.spawn\_rwvc[t]$\gets$max(U.wait\_rwvc[t],vc[t])
            %           \EndFor

            \EndProcedure

            \Function{CheckHB}{\epoch{c}{u},\task{T}}
            \State \Comment{Check HB between epoch \epoch{c}{u} and %current access by
                \task{T}'s access}
            \If{\epoch{c}{u} $\preceq$ \task{T.rw\_vc} \textbf{or} \epoch{c}{u} $\preceq$ \task{T.ro\_vc} \textbf{or} \task{u} $\in$ \task{T.joinset}}
            \State \Return true
            \EndIf
            \State \Return false
            \EndFunction

        \end{algorithmic}
    \end{algorithm}

    %\begin{algorithm}[H]
    %	\caption{\hfill \ft: \thr{T} acquires lock \thr{L}}
    %	\label{alg:ft-lockAcquire}
    %	\begin{algorithmic}[1]
    %		\ForAll{<t,c> in L.vc}
    %		\State T.vc[t] $\gets$ max(L.vc[t], T.vc[t])
    %		\EndFor
    %	\end{algorithmic}
    %\end{algorithm}
    %\begin{algorithm}[H]
    %	\caption{\hfill \ft: \thr{T} releases lock \thr{L}}
    %	\label{alg:ft-lockRelease}
    %	\begin{algorithmic}[1]
    %		\State L.vc $\gets$ T.vc
    %		\State T.m\_epoch $\gets$ T.m\_epoch + 1
    %	\end{algorithmic}
    %\end{algorithm}
\end{small}


==> nft-pseudocode.tex <==
\begin{small}
    \begin{algorithm}[H]
        \caption{\hfill \nft: \thr{T} spawns \thr{U}}
        \label{alg:nft-task-spawn-opt}
        \begin{algorithmic}[1]
            \If{\texttt{size}(\thr{T}.rw\_vc) $>$ THRESHOLD}
            \State \thr{T}.ro\_vc $\gets$ REF(\{\thr{T}.ro\_vc $\cup$ \thr{T}.rw\_vc\})
            \State \thr{T}.rw\_vc $\gets$ $\emptyset$
            \EndIf

            \State \thr{U}.ro\_vc $\gets$ \thr{T}.ro\_vc
            \State \thr{U}.rw\_vc $\gets$ \thr{T}.rw\_vc $\cup$ \{\thr{T}.epoch\}
            \State \thr{U}.joinset $\gets$ \thr{T}.joinset
            %                \State U.m\_rw\_vc $\gets$ T.m\_rw\_vc $\cup$ \{<T.taskid , T.clock>\}
            %           \State U.wait\_rovc $\gets$ T.spawn\_rovc
            %           \State U.wait\_rwvc $\gets$ T.spawn\_rwvc $\cup$ \{<T.taskid , T.clock>\}

            \swarnendu{Is incrementEpoch() different from just incrementing the clock value?}

            \State \algorithmiccomment{incrementEpoch() creates a new epoch with clock value incremented by 1}
            %  and returns its pointer}
            \State \thr{T}.epoch $\gets$ incrementEpoch(1)
            \State \thr{U}.epoch $\gets$ incrementEpoch(1)
        \end{algorithmic}
    \end{algorithm}
    \begin{algorithm}[H]
        \caption{\hfill \nft: \thr{T} joins with \thr{U}}
        \label{alg:nft-join-opt}
        \begin{algorithmic}[1]
            \State      \thr{T}.\pcode{joinset}  $\gets$ \thr{T}.\pcode{joinset} $\cup$ \{getTaskId(\thr{U}.epoch)\}
            \State \algorithmiccomment{getTaskId() returns task id of the corresponding epoch}
            %
            %           \ForAll{<t,c> in U.wait\_rwvc}
            %           \State vc $\gets$ \{T.wait\_rovc $\cup$ T.wait\_rwvc\}
            %           \State T.wait\_rwvc[t]$\gets$max(U.wait\_rwvc[t],vc[t])
            %           \State T.spawn\_rwvc[t]$\gets$max(U.wait\_rwvc[t],vc[t])
            %           \EndFor
        \end{algorithmic}
    \end{algorithm}
    \begin{algorithm}[H]
        \caption{\hfill \nft: HB\_Check(c@u,\thr{T})}
        \label{alg:nft-hb-check}
        \begin{algorithmic}[1]
            \If{c@u $\preceq$ \thr{T}.rw\_vc \textbf{or} c@u $\preceq$ \thr{T}.ro\_vc \textbf{or} u $\in$ \thr{T}.joinset }
            \State \textbf{return} true
            \EndIf
            \State \textbf{return} false
        \end{algorithmic}
    \end{algorithm}
    %\begin{algorithm}[H]
    %	\caption{\hfill \ft: \thr{T} acquires lock \thr{L}}
    %	\label{alg:ft-lockAcquire}
    %	\begin{algorithmic}[1]
    %		\ForAll{<t,c> in L.vc}
    %		\State T.vc[t] $\gets$ max(L.vc[t], T.vc[t])
    %		\EndFor
    %	\end{algorithmic}
    %\end{algorithm}
    %\begin{algorithm}[H]
    %	\caption{\hfill \ft: \thr{T} releases lock \thr{L}}
    %	\label{alg:ft-lockRelease}
    %	\begin{algorithmic}[1]
    %		\State L.vc $\gets$ T.vc
    %		\State T.m\_epoch $\gets$ T.m\_epoch + 1
    %	\end{algorithmic}
    %\end{algorithm}
\end{small}


==> nft.tex <==
% \section{Vector-Clock-Based Race Detection for Structured Task Parallelism\label{sec:nft-design}}
\section{Adapting Vector Clocks for %\pcode{Fork-Join}
  Task Parallelism\label{sec:nft-design}}

% In the previous section, we discussed challenges in \naively re-purposing a vector-clock-based data race detection algorithm like \ft for task parallel programs.

% \swarnendu{\nft works for unstructured task-based programs with fork-join parallelism, the child tasks need not join with the parent. It seems \cracer requires nested fork-join parallelism.}

In this section, we discuss our extensions to repurpose the %vector-clock-based
\ft data race detection algorithm~\cite{fasttrack2,fasttrack} for unstructured task-based programs.
% Our design, called \emph{\nft}, extends the \emph{\ft} algorithm~\cite{fasttrack2,fasttrack}.
% Whereas prior work has discounted the possibility of using vector clocks for task-based programs, this work aims to retarget vector clocks for efficient race detection of task-parallel programs.
Task-based programs create more, often more orders of magnitude, parallel tasks than threads in multithreaded programs.
% For example, the benchmarks evaluated in this work create
% a minimum of 150--300 tasks (for \blackscholes) and a maximum of $\sim 3 \times 10^{6}$ tasks (for \nn).
For example, the benchmark \nn
% evaluated in this work
creates up to $\sim 3 \times 10^{6}$ tasks (Table~\ref{tab:run-time-stats}).
% These are an order of magnitude greater than the multithreaded Java applications that are part of the popular DaCapo benchmark suite, which spawn \mindacapothreads--\maxdacapothreads threads.
% Techniques like \ft that track the happens-before relation use a per-thread and per-variable vector clock to encode the clock values of all threads in the system.
Techniques like \ft use a per-thread and per-variable vector clock to encode the clock values of all threads in the system. While this representation works fine for multithreaded programs where the number of concurrent threads is comparatively small
(\(\sim\)\#cores), it is impractical for task-based programs and leads our
% \naive\xspace
\ft implementation
to fail on several benchmarks because of memory overheads (Section~\ref{sec:eval:perf}). Storing
only the non-zero entries in a vector clock does not help since several concurrent tasks potentially access shared read-only variables.
%  at some point during the application.
\savespace{Whereas prior work has discounted using vector clocks for task-based programs~\cite{cracer-spaa-2016,ptracer-fse-2016,spd3-pldi-2012}, \nft shows how to achieve competitive performance
    % for generic unstructured task-based programs.
    with a curated set of optimizations.}

%% In the previous section, we discussed challenges in \naively re-purposing a vector-clock-based data race detection algorithm like \ft for task parallel programs. In this section we discuss our proposed optimizations to the basic \ft algorithm to adapt it to task parallel programs. Then in section 3.2 we discuss our proposed new algorithm for vector clock based race detection with constant memory metadata for variables even in case of multiple parallel readers.

% \input{ft-states.tex}

% \swarnendu{Give examples of the difference between threaded programs and task-parallel programs.}
% \input{threads-tasks.tex}

\savespace{\subsection{Optimized Per-Task Vector Clock Representation}}

% We profiled benchmarks for which \ft ran out of memory. 7 out of 11 of our benchmarks ran out of memory and failed to execute with \naive \ft.
% \hilite{XXX of our benchmarks ran out of memory and failed to execute with \naive \ft (Section~\ref{sec:eval})}.

% \paragraph*{Store nonzero entries.}
% \shivam{Do we want to retain this para? Storing non-zero entries isn't essentially an optimization}
% We observe that a single task synchronizes with few tasks during its lifetime, so most vector clock entries in a task remain zero. A simple solution is to store the non-zero entries in a vector clock, entries which are not present are assumed to have a clock value of zero.

% This optimization helped executing fasttrack on all of the benchmarks on our system, without any memory issues.

% \subsection{Optimized Vector Clock Representation for Tasks}

We analyzed the performance of \ft
% on benchmarks
and found that the task vector clock operations incur high time and space overhead.
% Specifically,
For example, the task join operation is a bottleneck because it requires
%  iterating and
comparing and merging all the clock values in the child and the parent tasks' vector clocks.
\Naively merging the vector clocks is not required since most vector clock entries remain unchanged during the lifetime of a task.
In the following, we discuss two novel optimizations employed in \nft.

% In \ft, \pcode{wait()} calls require a join of the vector clocks of the parent and the child tasks. This requires iterating over all the epoch values in the child's vector clock and merging them with the parent's vector clock.

\iftoggle{ieeeFormat}{
    % \input{nft-pseudocode-merged-algorithmic.tex}
    \input{nft-pseudocode-merged-algpseudocode.tex}
}{}

\iftoggle{acmFormat}{
    \input{nft-pseudocode-merged-algpseudocode.tex}
}{}

\paragraph*{Tracking read-only clock entries}

The first insight in \nft
is that \emph{most} vector clock entries for a task remain unchanged during the lifetime of the task, and the clock values continue to be the same as in the parent task. Thus, maintaining per-task copies of the clock entries is mostly redundant.
%  and rarely required.

% Almost all vector clock entries for a task remain unchanged during the lifetime of the task and the epoch values are same as in the parent task. Thus, maintaining per-task copies of the vector clocks are redundant and are rarely required. This motivated us to store a reference to a read-only parent vector clock \pcode{rovc} from the child task, instead of explicitly copying the epoch values from parent to the child.

% \swarnendu{Shivam: What is the intuition to merge to a \pcode{ro\_vc} when the size is large? We should also say what will happen when an entry in the \pcode{ro\_vc} is modified.}

In \nft, the vector clock of a task is partitioned into a read-only (denoted by \pcode{ro\_vc}) and a read-write portion (denoted by \pcode{rw\_vc}). Child tasks in \NFT maintain a reference to the read-only vector clock  \pcode{ro\_vc} of their parents instead of maintaining redundant copies.
% of the clock values.
During a \pcode{spawn} operation (\pcode{\smaller SPAWN}, Algorithm~\ref{alg:nft-sync-ops}), \nft first checks if the size of \pcode{rw\_vc} is greater than a threshold. If yes, then
\nft merges \pcode{ro\_vc} and \pcode{rw\_vc} of the parent task into a new \pcode{ro\_vc} for the child task and \pcode{rw\_vc} of child task is kept empty.
% MAX\_VC\_SIZE,
Otherwise, the child \pcode{ro\_vc} points to the parent \pcode{ro\_vc} and the
parent's \pcode{rw\_vc} is copied to the child's \pcode{rw\_vc}.
% This reduces the redundancy significantly since now complete vector clock copies happen only when the size of \pcode{rw\_vc} is greater than \pcode{\smaller THRESHOLD}. In the common case, most vector clock entries of a task remain unchanged, \ie, the size of \pcode{rw\_vc} is small.
% the contents of
Therefore, maintaining read-only portions of the vector clocks reduces space overheads and improves performance by avoiding needless copies and operations on redundant clock values. Complete vector clock copies happen only when the size of \pcode{rw\_vc} is greater than \pcode{\smaller THRESHOLD}. In the common case, most vector clock entries of a task remain unchanged, \ie, the size of \pcode{rw\_vc} is small.

% \swarnendu{SK: Can you create a small example with concrete or symbolic clock values, like the SlimFast~\cite{slimfast} examples?}

% \swarnendu{Is the following argument valid: ``In a \pcode{wait} call, \nft needs to merge just the epoch values present in \pcode{rw\_vc} of the child task.''?}

% Task vector clock is divided into a \emph{read-only} part and a \emph{read-write} part. Tasks maintain a reference of the read-only part and the reference is updated and passed to children as appropriate. During a \pcode{spawn}, \nft first checks if size of \pcode{rwvc} is less than a threshold,
% MAX\_VC\_SIZE,
% otherwise \nft merges \pcode{rovc} and \pcode{rwvc} into a new \pcode{rovc} and clears the contents of \pcode{rwvc}. Thereafter, \nft copies the \pcode{rwvc} of the parent task to \pcode{rwvc} of the child task and the child \pcode{rovc} is made to reference at the parent \pcode{rovc}. Thereby, the redundancy of the vector clock entries is significantly reduced, improving performance.

%
%During a \pcode{spawn()} function, it is desirable for the vector clock of the parent task to be small, to reduce the memory overhead and data redundancy due to multiple copies of the same data. In \ft, \pcode{wait()} calls require a join of the vector clocks of the parent and the child tasks. This requires iterating over all the epoch values in the child's vector clock and merging them with the parent's vector clock. However, since most of the epoch values remain unchanged during the lifetime of a task, \naively merging the complete vector clocks is unneeded. To optimize the overhead of \pcode{wait}, we need to store only the modified epoch values in a task's vector clock. This may however break the first requirement, \ie, the size of a vector clock should be
%small, since the size of the modified clock entries can be large in rare cases.
%
%% less than MAX\_VC\_SIZE , as the size of modified epoch values can always grow large than this.
%In order to resolve this, \nft adopts a ``double vector clock'' structure. In the double representation, \nft stores two vector clocks per task, \pcode{spawn\_vc} and \pcode{wait\_vc}, where each target the \pcode{spawn} and \pcode{wait} optimization requirements respectively.
%% In order to incorporate the optimizations,

%Every task maintains two references: \pcode{spawn\_rovc} and \pcode{wait\_rovc} and two actual vector clocks: \pcode{spawn\_rwvc} and \pcode{wait\_rwvc}.  Here, \pcode{wait\_rwvc} contains all the epoch values modified during the lifetime of a task, and \pcode{wait\_rovc} is a reference to the unmodified epoch values. On the other hand, \pcode{spawn\_wrvc} is used to help optimize the memory overhead of task spawn. The size of \pcode{spawn\_wrvc} is kept small and the rest of the epoch values are referenced through \pcode{spawn\_rovc}.
%Note that the two vector clocks \pcode{spawn\_rovc} and \pcode{wait\_rovc} are identical overall, \ie, the same epoch values are present in both of them. Figure~\ref{fig:metadata-states} describes the task metadata structure used in \ft and \nft.
% In the spawn call, we want our parent TaskVc to be small,say less than MAX\_VC\_SIZE, to reduce memory overhead and data redundancy due to multiple copies of same data. In \ft, wait calls as well incur high runtime overhead, as we need to iterate over all the epoch values in child VC and merge them to the parent VC. However, since most of the epoch values remain unchanged in the  lifetime of the task, merging them is useless. So, to optimize the wait time overhead, we need to store only the modified epoch values in TaskVC. This however contradicts our first requirement i.e. size of a TaskVC shoukd be less than MAX\_VC\_SIZE , as the size of modified epoch values can always grow large than this.

%Figure~\ref{fig:metadata-states} describes the task metadata structure used in \ft and \nft. \ft uses a single vector clock for storing the epoch values of \emph{all} other tasks. In order to optimize both time and space, \nft adopts a ``double vector clock'' structure. In a double representation, having two vector clocks, \pcode{vc} and \pcode{child\_vc}, where each of them has two parts: \emph{read-only} \pcode{ro\_root\_vc} and \emph{read-write} \pcode{rw\_vc}. \pcode{rw\_vc} contains all the epoch values modified during the lifetime of a task, and \pcode{ro\_root\_vc} is a reference to the unmodified epoch values. In a \pcode{wait} call, \nft needs to merge just the epoch values present in \pcode{rw\_vc} of the child task. On the other hand, \pcode{child\_vc} is used to help optimize the memory overhead of task spawn.
%The size of \pcode{rw\_vc} in the \pcode{child\_vc} is usually small,
%%  always be less than MAX\_VC\_SIZE,
%and the rest epoch values are referenced through the \pcode{ro\_root\_vc} component in \pcode{child\_vc}. Note here, that overall the two vector clocks are identical, \ie, the same epoch values are present in both of them.
%
%\swarnendu{SK: Update \nft metadata in Figure~\ref{fig:metadata-states}. The description and the figures are inconsistent.}
% Task vector clock is divided into a \emph{read-only} part and a \emph{read-write} part. Tasks maintain a reference of the read-only part and the reference is updated and passed to children as appropriate. During a \pcode{spawn}, \nft first checks if size of \pcode{rwvc} is less than a threshold,
% % MAX\_VC\_SIZE,
% otherwise \nft merges \pcode{rovc} and \pcode{rwvc} into a new \pcode{rovc} and clears the contents of \pcode{rwvc}. Thereafter, \nft copies the \pcode{rwvc} of the parent task to \pcode{rwvc} of the child task and the child \pcode{rovc} is made to reference at the parent \pcode{rovc}. Thereby, the redundancy of the vector clock entries is significantly reduced, improving performance.

%
% During a \pcode{wait}, since \pcode{wait\_rwvc} of child task contains the modified epoch values, \nft merges it to parent \pcode{wait\_rwvc} and \pcode{sapwn\_rwvc}.

% , even after having data redundancy in VC and childVC.

% \swarnendu{Draw a figure, give an example.}
% \shivam{Which sort of figure?}

% We observe that this optimization alone reduces the space and performance overhead significantly.

% In \ft size of vector clock increases majorly when two tasks join.
% % which only happens after a wait(), wait\_for\_all(), lock\_acquire() or lock\_relese() operation.
% So in join operation we check if size of task vector clock is more than a
% maximum limit, if so we make an \emph{read-only} vector clock  \pcode{root\_vc}, which contains all the entries of the
% task vector clock and the task vector clock is reset to be empty. All descendant tasks of this task maintain
% a reference to the \pcode{root\_vc} and follow the copy-on-write mechanism. In this way after a join the vector clock of
% a task will only contain entries it modifies or frequently use and all other entries are in \pcode{root\_vc}.
% So any task $T$'s vector clock only contains (i) entries copied from parent’s vector clock, or (ii) entries that have
% been modified by $T$, or  (iii) new entries corresponding to child tasks created by $T$ before a join operation.
% So effectively $T$'s vector clock is the combination of its current vector clock and \pcode{root\_vc}. Whenever a task perform vector clock operations,
% %(\ie, requires looking up clocks of tasks not present in their vector clocks),
% it checks with the read-only \pcode{root\_vc} vector clock. We observe that this optimization alone reduces the space
% and performance overhead significantly.

% We use the popular Copy-on-Write (CoW) mechanism to optimize the vector clock representations for child tasks.
% Each root task in the task graph maintains a \emph{read-only} vector clock. Whenever a root task is spawned,
% a new vector clock \pcode{root\_vc}, which is a copy of the parent’s vector clock, is created. All descendant
% tasks of the new root task maintain a reference to the \pcode{root\_vc} and follow the copy-on-write mechanism,
% so any task $T$'s vector clock only contains (i) entries that have been modified by $T$, or (ii) new entries
% corresponding to child tasks created by $T$ \hilite{or their ancestors after corresponding root}. Whenever a
% task perform vector clock operations,
% %(\ie, requires looking up clocks of tasks not present in their vector clocks),
% it checks with the read-only \pcode{root\_vc} vector clock. This optimized representation helps reduce the
% overhead of every vector clock operation from \bigO{n} to just the number of entries that are actually modified.
% We observe that this optimization alone reduces the space and performance overhead significantly.

\paragraph*{Optimizing vector clock join}

% \sout{Task parallel programs can spawn thousands of tasks which leads to vector clocks with large number of entries for each task.
%   This leads to high time and memory overhead for task metadata operations in \ft.}
% Furthermore, \ft maintains per-variable and per-task metadata in the form of vector clocks.
% Having a large number of tasks also increases the memory overhead substantially.
% , which also contributes to performance overhead.

% Child tasks that join with their parent tasks complete before the join operation.
% % are no longer alive.
% Subsequent access to any shared variable by the parent task always happens after the child task's accesses.
An access to a shared variable by a parent task after joining with a child task always happens after the child's accesses, since the accesses are synchronized by the \pcode{join} operation.
The second insight in \nft is that
% Therefore
it does not need to store the clock values of the child tasks \emph{after} the join operation. Instead, tracking the set of all child tasks that have joined with the parent task suffice.
% This can be done efficiently using better data structures, thereby reducing the \pcode{join} overhead significantly.

% It should be noted here that child tasks which have already joined with parent tasks must have completed before the join operation and so are no longer live. Therefore, subsequent accesses to any shared variable by the parent task will always have happens-after relationship with the access by the  child tasks accesses. And therefore, we don't essentially need to store the clock values of all these children tasks. Instead just a set of all such tasks, which have joined with parent task, will suffice.

% We use the same idea for optimizing the \pcode{join} operation in \nft.

%Each task in \nft maintains the set of child tasks which have already joined with it in a \pcode{joinset} data structure. When a parent task joins with a new child task, the child task is added to the \pcode{joinset} of the parent task.(See Algorithm~\ref{alg:nft-join-opt}) During an access of a shared variable \pcode{x}, \nft checks if the tasks contained in the access history of \pcode{x} are present in the \pcode{joinset}. If all the tasks are present in the \pcode{joinset}, then \nft infers that the current access to \pcode{x} happens \emph{after} the past accesses. This allows \nft to avoid expensive vector clock updates for join operations,
%% without breaking the semantics of \ft
%without compromising on correctness.(See Algorithm~\ref{alg:nft-hb-check})

Each task in \nft maintains the set of child tasks that have already joined with it in a \pcode{joinset} data structure.
No vector clock join occurs when a task \task{T} joins with task \task{U},
% When the parent task joins with a child task, the child task is added to the \pcode{joinset} of the parent task (\pcode{\small JOIN}, Algorithm~\ref{alg:nft-sync-ops}).
instead, the child task is added to the \pcode{joinset} of the parent task (\pcode{\smaller JOIN}, Algorithm~\ref{alg:nft-sync-ops}).
When a parent task spawns a new child task, the parent \code{joinset} is copied to the child \code{joinset}.
%  (\pcode{\small SPAWN}, Algorithm~\ref{alg:nft-sync-ops}).

Algorithm~\ref{alg:ft-sync-ops} shows that the complete vector clock is used for all the task operations in \ft, which is expensive and often unnecessary. Algorithm~\ref{alg:nft-sync-ops} shows the optimized spawn and join algorithms in \nft. \nft uses the same algorithm for lock acquire and release as \ft.

The \nft algorithm to check for the happens-before relation between prior accesses and the current access needs to be modified not to compromise correctness. Before accessing a shared variable \pcode{x}, \ft compares the current task vector clock with the epoch(s) stored in \pcode{x}'s access history to determine if current access to \pcode{x} happens \emph{after} the past accesses (\pcode{\smaller CHECKHB}, Algorithm~\ref{alg:nft-sync-ops}). \nft, apart from the vector clock entry check, also checks if the tasks present in \pcode{x}'s access history belong to the \pcode{joinset} of the current task. If all the tasks are present in the \pcode{joinset}, \nft infers that the current access %to \pcode{x}
happens \emph{after} the prior accesses.
% Algorithm~\ref{alg:nft-sync-ops} shows how \nft checks for the happens-before relation between an epoch and the current access in a task.
Since the vector clock is spread across %three parts
\code{ro\_vc}, \code{rw\_vc}, and \code{joinset} in \nft, \pcode{\smaller CHECKHB} checks the HB relation against all of them.
% We do not show the last optimizations, vector clock caching, reduce redundancy of epoch metadata, and state specialization, to avoid clutter.

% This allows \nft to avoid expensive vector clock updates for \pcode{join} operations without compromising on correctness.

% Every task contains a set of child tasks which have already joined with it i.e. \textit{joinset}. If the parent task joins with a new child task, the child task is added to the joinset of parent task. In any shared access, the detector checks that if the tasks contained in the access history of the shared variable are there in joinset, if yes it infers that the current access has happens after relationship with the past access. Therefore we successfully avoid task vector clock updations in case of join operation, without breaking the semantics of \ft.

The size of task vector clocks reduces significantly due to the \pcode{joinset} optimization. Note that a trivial implementation of the \pcode{joinset} may not give performance benefits over \ft. We use efficient set implementations based on the Union-Find data structure, which reduces the overhead of set operations.

% \paragraph*{Algorithmic details.}

% Vector$<$parent\_clocks$>$: The vector of parent\_clock is an immutable structure created only during the creation
%of task.It contains the relative position of the task in the corresponding task graph.\\

% List$<$child$>$: It stores the list of children of a task.\\

% Varstate\{\\
% List $<$Lockstate\_entry$>$;\\
% \}\\
% Here, each variable maintains a list of entries, where each entry correspond to a given lockstate with which the variable was accessed.These entries are of constant size and are as follows:\\
% Lockstate\_entry\{\\
% Lockset LS;\\
% Read\_epoch r1;\\
% Pointer pr1;\\
% Read\_epoch r2;\\
% Pointer pr2;\\
% Write\_epoch w1;\\
% Pointer pw1;\\
% Write\_epoch w2;\\
% Pointer pw2;\\
% \}\\

\paragraph*{Vector clock caching}
%
%\shivam{Should it be kept here or in implementation section?}
% \swarnendu{SK: What is the data structure previously and what does the data structure look like after caching? Please provide more details for me to revise. Adding a diagram for the paper might be good.}

The size of vector clocks for a few tasks can still be large even after the above optimizations.
% Accessing the vector clock data structure at every shared memory access can lead to overhead.
\nft caches few clock entries with variable placeholders, using a sliding window approach, to further improve the performance. Profiling the access times of such task vector clocks show % significant
improvement post the caching optimization.

% Accessing the vector clock data structure in every access adds overhead. To reduce this, first few entries of the vector clock can be cached in the taskstate itself to improve common-case access time. On profiling, it was observed that the after caching, the vector clock data structure access was significantly low, improving performance.

\paragraph*{Race detection}

% Please note the fact that all the optimizations discussed hereby are on the top of \ft i.e. \nft is essentially \ft plus these  optimizations. For a better understanding of \ft, refer Section \ref{sec:ft}.

The steps to update metadata and detect races in \nft extend the \ft algorithm (Section~\ref{sec:ft}).
For every shared variable, \nft stores one write epoch to track the last write access. The read metadata varies between an epoch and a complete vector clock, as in \ft.
% If there are multiple concurrent readers, the read metadata is stored as vector clock otherwise epoch corresponding to only last read access is stored.
When a shared variable is accessed, \nft checks if all previous
% potentially conflicting
accesses happen before the current access using \pcode{\smaller{CHECKHB}} (Algorithm~\ref{alg:nft-sync-ops}).
% If yes, the metadata is updated accordingly i.e. for write access, write epoch is updated and for read access, read metadata is updated depending on whether it is {\small READ-EXCLUSIVE, READ-SHARE or READ-SHARED} case(\cite{fasttrack}).
% Otherwise a data race is reported.
If yes, then the metadata is updated; otherwise, a data race is reported.
% \sout{For a write access, all previous accesses are potentially conflicting, while for a read access, only the previous write could conflict.}
Like \ft, \NFT is also dynamically sound and precise.

% \begin{figure}
%     \centering
%     % \includegraphics{slimfast}
%     \caption{Metadata redundancy across accesses in release-free regions of code.}
%     \label{fig:slimfast-opts}
% \end{figure}

\savespace{Figure~\ref{fig:metadata-states} compares the metadata maintained in \ft and \nft. Given a task \task{T}, a \naive \ft algorithm uses a single vector clock representation for storing the epoch values of \emph{all} other tasks (\code{vc} in \code{PerTaskMetadata}). As discussed, \nft adopts a ``double vector clock'' structure, with a read-only part and a read-write part, to optimize both time and space.}

% Algorithms~\ref{alg:ft-task-spawn-unopt} and \ref{alg:ft-join-unopt} show the unoptimized spawn and join algorithms in \ft. In \ft, the whole vector clock with non-zero clock entries is used for all the task operations which is expensive and often unnecessary. Algorithms~\ref{alg:nft-task-spawn-opt} and \ref{alg:nft-join-opt} show the optimized spawn and join algorithms in \nft. The \nft algorithms show the two optimizations, optimizing joins and maintaining read-only vector clocks, which are new contributions in this work.

% Algorithms ~\ref{alg:ft-lockAcquire} and ~\ref{alg:ft-lockRelease} show the lock acquire and lock release algorithms, respectively, in \ft. \nft also uses the same algorithm for lock acquire and release.
% % , so we haven't shown them separately.

% \paragraph*{Reduce redundancy of epoch metadata}

% % Prior work, called \emph{SlimFast}, has proposed techniques to reduce the redundancy in tracking metadata in the \FT algorithm~\cite{slimfast}.

% All shared variables updated by a task \task{T} in a release-free region\footnote{Release-free regions are per-thread dynamic code regions demarcated only by synchronization release operations such as lock releases, monitor wait, and thread fork.} (RFR) will have the same epoch value. For example, writes to \pcode{x} and \pcode{y} by task \task{T} in the same RFR result in the same epoch value as the write metadata for both \pcode{x} and \pcode{y}. Inspired by prior work called \emph{SlimFast}~\cite{slimfast} that reduces metadata redundancy in \ft, each task in \NFT maintains an immutable epoch value and increments it only after a synchronization release operation. When \nft needs to update the write epoch of a variable \pcode{x}, it makes \pcode{x}'s write metadata to point to \task{T}'s immutable epoch.
% \savespace{The write epoch optimization is valid in all the three write states in \ft (see Table~\ref{tab:ft-states}).
%     The read epoch optimizations are applicable for reads in the \rdsameepoch and \rdexclusive states.}
% % We apply optimizations of epoch metadata from prior work~\cite{slimfast}.  All the writes by a task t within a given epoch result in the same epoch value for the variables write epochs.
% % To eliminate redundant metadata for such accesses, every task maintains an immutable epoch.
% % Whenever a variable x needs epoch update, x's epoch is set directly to t's epoch. Task t's epoch is updated on Release and Fork operations.
% % The third case is to avoid redundancy for read metadata that are in the form of vector clocks.
% We ignore redundancy in read vectors since
% % the optimization of
% using a separate representation for read-only vectors proves effective.

% The \FT data race detection algorithm suffers from metadata redundancies~\cite{slimfast,slimstate}.
% % Prior work has observed different sources of metadata redundancy in
% % % a vector-clock-based
% % the \ft data race detection algorithm~\cite{slimfast,slimstate}.
% \citet{slimfast} discuss optimizations to address redundancy in tracking write epochs, read epochs, and read vector clocks. In the write epoch case, all variables updated by a task \task{T} in a release-free region\footnote{Release-free regions are per-thread dynamic code regions demarcated only synchronization release operations such as lock releases, monitor wait, and thread fork.} (RFR) will have the same epoch value.
% For example, within an epoch, writes to \pcode{x} and \pcode{y} result in the same epoch value as the write metadata for both \pcode{x} and \pcode{y}.
% % (shown in Figure~\ref{fig:slimfast-opts}).
% Each task in \NFT maintains an immutable epoch value, which is updated after every synchronization release operation. When \nft needs to update the write epoch of a variable \pcode{x}, it makes \pcode{x}'s write metadata point to \task{T}'s immutable epoch. The write epoch optimization is valid in all the three write states in \ft (see Table~\ref{tab:ft-states}). The read epoch optimizations are similar, and are applicable for reads in the \rdsameepoch and \rdexclusive states.
% % We apply optimizations of epoch metadata from prior work~\cite{slimfast}.  All the writes by a task t within a given epoch result in the same epoch value for the variables write epochs.
% % To eliminate redundant metadata for such accesses, every task maintains an immutable epoch.
% % Whenever a variable x needs epoch update, x’s epoch is set directly to t’s epoch. Task t’s epoch is updated on Release and Fork operations.
% The third case is to avoid redundancy for read metadata that are in the form of vector clocks. We ignore redundancy in read vectors since the optimization of using a separate representation for read-only vectors prove effective.

\savespace{
    \input{tab-nft-rules.tex}
}

% \paragraph*{Optimizing tracking shared readers}

% Prior extensions to \ft avoid redundant updates to read vector entries when the current clock of the reader thread \thr{T} matches the clock when \thr{T} last read the variable~\cite{fasttrack2,fib-oopsla-2017,valor-oopsla-2015}. The fast path optimization is applicable to $\sim$35\% of all read accesses (average across all benchmarks), which shows that read shared state specialization is important for task-based programs.

% Prior work show that specializing the \rdshared states in \ft can improve performance for
% multithreaded programs~\cite{fasttrack2,fib-oopsla-2017,valor-oopsla-2015}. The \rdsharedsameepoch state in \nft avoids redundant updates for read vector entries when the current clock of the reader thread \thr{T} matches the clock when \thr{T} last read the variable. Table~\ref{tab:rules} shows the breakdown of memory accesses (average across all benchmarks) for task-based programs (see Section~\ref{sec:eval:setup}) into different \nft states. We find that $\sim$35\% of all read accesses are to the \rdsharedsameepoch state, which shows that read state specialization is useful even for task-based programs.

% We borrow the idea of specializing read states in \ft from prior
% work~\cite{valor-oopsla-2015,fasttrack2,fib-oopsla-2017}. The \rdsharedsameepoch state avoids
% redundant updates for read vector entries when the current clock of the reader thread \thr{T}
% matches the clock when \thr{T} last read the variable. Table~\ref{tab:rules} shows the breakdown
% of memory accesses (average across all benchmarks) into different \ft states. In our experiments,
% we found $\sim$35\% of all read accesses are to the \rdsharedsameepoch state which shows the
% importance of the state specialization optimization.

% A large fraction of read accesses are \rdsharedsameepoch which shows  the importance of the state
%  specialization optimization. for task parallel programs. We observe a non-trivial performance
%  benefit after applying the optimization to task parallel programs (Section~\ref{sec:eval}).

% \subsection{Pseudocode}

\savespace{
    \input{fig-ft-nft-state.tex}
}

% \swarnendu{Summarize and describe the main differences between \ft and \nft. An option is to move the discussion to the relevant optimizations instead of having a separate section.}

% Figure~\ref{fig:metadata-states} compares the metadata maintained in \ft and \nft. Given a task \task{t}, a \naive \ft algorithm uses a single vector clock representation for storing the epoch values of \emph{all} other tasks (\code{m\_vc} in \code{PerTaskMetadata}).
% \nft adopts a ``double vector clock'' structure, with a read-only part and a read-write part, to optimize both time and space.


% Algorithms~\ref{alg:ft-task-spawn-unopt} and \ref{alg:ft-join-unopt} show the unoptimized spawn and join algorithms in \ft. In \ft, the whole vector clock with non-zero clock entries is used for all the task operations which is expensive, and unnecessary. Algorithms~\ref{alg:nft-task-spawn-opt} and \ref{alg:nft-join-opt} show the optimized spawn and join algorithms in \nft. The \nft algorithms show the two optimizations, optimizing joins and maintaining read-only vector clocks, which are new contributions in this work. We do not show the last optimizations, vector clock caching, reduce redundancy of epoch metadata, and state specialization, to avoid clutter.

\medskip

\noindent The optimizations discussed substantially improve the time and space overheads of \nft for task-based programs. We emphasize that \nft analysis is generic,
% works for unstructured task-based programs that use fork-join parallelism or locks for synchronization.
\eg, like \ft, it can analyze unstructured task-based programs and programs with lock-based synchronization.
% \shivam{There is no discussion regarding race detection algorithm fo FastRacer. The reader would have no idea how data race detection happens in \nft}
% Section~\ref{sec:eval} shows that \nft  is competitive with prior work which target \emph{only} structured \pcode{async-finish} programs.

% The above extensions to \ft improve the run-time and space overhead of \nft for unstructured task-based programs. Section~\ref{sec:eval} shows that \nft is competitive with prior work which \emph{target} structured \pcode{async-finish} programs.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> tab-benchmarks.tex <==
\begin{table}
    \centering
    \begin{tabular}{lll}
        \textbf{Application}  & \textbf{Benchmark Suite}       & \textbf{Input} \\
        \toprule
        \bench{blackscholes}  & PARSEC~\cite{parsec-pact-2008} & native         \\
        % \bench{bodytrack}     & PARSEC~\cite{parsec-pact-2008} &                \\
        \bench{fluidanimate}  & PARSEC~\cite{parsec-pact-2008} & native         \\
        \bench{streamcluster} & PARSEC~\cite{parsec-pact-2008} & large          \\
        \bench{swaptions}     & PARSEC~\cite{parsec-pact-2008} & small          \\
        \midrule
        \bench{convexHull}    & PBSS~\cite{pbbs-benchmarks}    &                \\
        \bench{delRefine}     & PBSS~\cite{pbbs-benchmarks}    &                \\
        \bench{delTriang}     & PBSS~\cite{pbbs-benchmarks}    &                \\
        \bench{nearestneigh}  & PBSS~\cite{pbbs-benchmarks}    &                \\
        \bench{rayCast}       & PBSS~\cite{pbbs-benchmarks}    &                \\
        \midrule
        \bench{karatsuba}     & SPP~\cite{spp-book}            &                \\
        \bench{kmeans}        & SPP~\cite{spp-book}            &                \\
        \bench{sort}          & SPP~\cite{spp-book}            &                \\
    \end{tabular}
    \swarnendu{This table does not seem to be super interesting. We can leave it out.}
    \caption{Details about the applications used in the evaluation. The inputs to the PARSEC benchmarks use the inputs provided with PARSEC, while the other benchmarks use the inputs provided in the public implementation of \ptracer.}
    \label{tab:benchmarks}
\end{table}


==> tab-nft-rules.tex <==
\iffalse
    \begin{table}
        \begin{subtable}{0.45\textwidth}
            \centering
            \begin{tabular}{llll}
                \textbf{\FT State}      & \textbf{Percentage} \\
                \toprule
                Read Same Epoch:        & 24.29               \\
                Read shared same epoch: & 35.10               \\
                Read exclusive:         & 32.50               \\
                Read shared:            & 7.56                \\
                Read share:             & 0.55                \\
                %Racy reads:             & 12.34               \\
            \end{tabular}
            \caption{Read rules.}
        \end{subtable}

        \begin{subtable}{0.45\textwidth}
            \centering
            \begin{tabular}{llll}
                Rule              & Percentage \\
                \toprule
                Write Same Epoch: & 20.21      \\
                Write exclusive:  & 73.25      \\
                Write shared:     & 6.54       \\
                %Racy writes:      & 15.44      \\
            \end{tabular}
            \caption{Write rules.}
        \end{subtable}
        \caption{Different rules used in benchmarks.}
        \label{tab:nft-rules-old}
    \end{table}
\fi

\begin{small}
    \begin{table}
        \centering
        \begin{tabular}{lr}
            \textbf{\NFT State} & \textbf{Accesses (\%)} \\
            \toprule
            \rdsameepoch        & 24.29                  \\
            \rdsharedsameepoch  & 35.10                  \\
            \rdexclusive        & 32.50                  \\
            \rdshared           & 7.56                   \\
            \rdshare            & 0.55                   \\
            % Racy reads:             & 12.34               \\
            % \midrule
            % \ftstate{Total}    & 100                 \\
            % \midrule
            \midrule
            \wrsameepoch        & 20.21                  \\
            \wrexclusive        & 73.25                  \\
            \wrshared           & 6.54                   \\
            % Racy writes:                     & 15.44               \\
            \bottomrule
            % \ftstate{Total}    & 100                 \\
        \end{tabular}
        % \swarnendu{AA: The non-racy reads + racy reads add up to 101\%. Please check.}
        % \swarnendu{AA: For this table, please scale non-racy reads to 100\%, \ie, ignore racy accesses.}
        % \swarnendu{Is the data correct and up to date?}
        % \swarnendu{We can use minipage to reduce the vertical space. Can we integrate this table with other floats?}
        \caption{Breakdown of reads and writes into different \nft states. The proportion of accesses in each state is an average over all benchmarks (Section~\ref{sec:eval}).}
        \label{tab:nft-rules-new}
    \end{table}
\end{small}


==> tab-runtime-stats.tex <==
\begin{table*}
    \centering
    \begin{tabular}{l|c|cccccc|cccc}
                       & \textbf{Memory} & \multicolumn{6}{c|}{\textbf{Reads}} & \multicolumn{4}{c}{\textbf{Writes}}                                                                           \\
        \cline{3-8}
        \cline{9-12}
                       &                 & Same                                & Shared Same                         & Exclusive & Shared & Share & Total & Same  & Exclusive & Shared & Total \\
                       &                 & Epoch                               & Epoch                               &           &        &       &       & Epoch &           &                \\
        \toprule
        \blackscholes  &                 &                                     &                                     &           &        &       &       &                                    \\
        \bodytrack     &                 &                                     &                                     &           &        &       &                                            \\
        \fluidanimate  &                 &                                     &                                     &           &        &       &       &       &                            \\
        \streamcluster &                 &                                     &                                     &           &        &       &       &                                    \\
        \swaptions     &                 &                                     &                                     &           &        &       &       &                                    \\
        \midrule
        \convexhull    &                 &                                     &                                     &           &        &       &       &       &                            \\
        \delrefine     &                 &                                     &                                     &           &        &       &       &                                    \\
        \deltriang     &                 &                                     &                                     &           &        &       &                                            \\
        \nn            &                 &                                     &                                     &           &        &       &       &                                    \\
        \raycast       &                 &                                     &                                     &           &        &       &       &                                    \\
        \midrule
        \kmeans        &                 &                                     &                                     &           &        &       &       &                                    \\
        \karatsuba     &                 &                                     &                                     &           &        &       &       &       &                            \\
        \sort          &                 &                                     &                                     &           &        &       &                                            \\
    \end{tabular}
    \swarnendu{Fill this in.}
    \caption{Run-time statistics of memory accesses across the different benchmarks.}
    \label{tab:runtime-stats}
\end{table*}


==> threads-tasks.tex <==
\begin{table*}[htbp]
    \centering
    \begin{tabular}{lc}
        \blackscholes  & \\
        \bodytrack     & \\
        \fluidanimate  & \\
        \streamcluster & \\
        \swaptions     & \\
        \midrule
        \convexhull    & \\
        \delrefine     & \\
        \deltriang     & \\
        \nn            & \\
        \raycast       & \\
        \midrule
        \kmeans        & \\
        \karatsuba     & \\
        \sort          & \\
    \end{tabular}
    \Description{A comparison of the number of threads spawned and the number of tasks across popular benchmarks used for data race detection.}
    \caption{A comparison of the number of threads spawned and the number of tasks across popular benchmarks used for data race detection.}
    \label{tab:threads-vs-tasks}
\end{table*}

